ASR-FAIRBENCH: Measuring and Benchmarking Equity Across Speech Recognition Systems

Automatic Speech Recognition (ASR) systems have become ubiquitous in everyday applications, yet significant disparities in performance across diverse demographic groups persist. In this work, we introduce the ASR-FAIRBENCH leaderboard which is designed to assess both the accuracy and equity of ASR models in real-time. Leveraging the Meta's Fair-Speech dataset, which captures diverse demographic characteristics, we employ a mixed-effects Poisson regression model to derive an overall fairness score. This score is integrated with traditional metrics like Word Error Rate (WER) to compute the Fairness Adjusted ASR Score (FAAS), providing a comprehensive evaluation framework. Our approach reveals significant performance disparities in SOTA ASR models across demographic groups and offers a benchmark to drive the development of more inclusive ASR technologies.

==> Application_Overview.tex <==
\section{Application overview}

The \textbf{ASR-FAIRBENCH} leaderboard is a web-based platform designed for evaluating and ranking ASR models. Built with React.js, leveraging an NVIDIA T4 GPU for inference, it offers an interactive platform for model submissions, performance analysis, and real-time leaderboard tracking. The platform is fully reproducible from its  repository\footnote{https://github.com/SatyamR196/ASR-FairBench}. The live leaderboard\footnotemark[\value{footnote}] can be accessed by users to submit their ASR models and receive an audit within minutes. The platform offers intuitive graphical representations of results, including box plots and histograms as shown in Figure \ref{fig:ui_features}, making it easier to interpret model performance.


% \begin{table} 
%     \centering
%     \small
%     \renewcommand{\arraystretch}{1.2}
%     \resizebox{\linewidth}{!}{ % Resize table to fit if needed
%     \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
%         \hline
%         \textbf{Model Name} & \textbf{ASR Score} & \textbf{WER} & \textbf{RTFX} & \textbf{Fairness Score} & \textbf{Gender} & \textbf{First Lang.} & \textbf{Socioecon.} & \textbf{Ethnicity} \\
%         \hline
%         openai/whisper-medium & 29.41 & 0.06 & 0.13 & 56.57 & 59.42 & 90.53 & 12.16 & 64.16 \\
%         openai/whisper-tiny   & 24.25 & 0.24 & 0.13 & 64.78 & 44.05 & 92.68 & 40.14 & 82.23 \\
%         facebook/wav2vec2-large-960h & 20.51 & 0.43 & 0.03 & 48.56 & 54.49 & 70.89 & 20.31 & 48.53 \\
%         facebook/hubert-large-ls960-ft & 20.31 & 0.40 & 0.03 & 42.94 & 12.75 & 88.91 & 14.92 & 55.18 \\
%         facebook/wav2vec2-base-960h & 19.82 & 0.48 & 0.66 & 45.86 & 14.58 & 77.01 & 31.06 & 60.77 \\
%         \hline
%     \end{tabular}}
%     \caption{Comparison of ASR Models Based on Performance and Fairness Metrics}
%     \label{tab:asr_comparison}
% \end{table}



\begin{figure}
    \centering
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth, height=4.8cm, keepaspectratio]{images/leaderboard.pdf}
        \caption{\textbf{ASR-FAIRBENCH} leaderboard}
        \label{fig:submit_model}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/Summary_with_FAAS3.pdf}
        \caption{Summarized results view.}
        \label{fig:summary_results}
    \end{subfigure}
    \caption{Key UI features: \textbf{ASR-FAIRBENCH} leaderboard, result summary, and performance analysis for whisper-small.}
    \label{fig:ui_features}
\end{figure}




